PROVES: Establishing Image Provenance using Semantic Signatures

Modern AI tools, such as generative adversarial networks, have transformed our ability to create and modify visual data with photorealistic results. However, one of the deleterious side-effects of these advances is the emergence of nefarious uses in manipulating information in visual data, such as through the use of deep fakes. We propose a novel architecture for preserving the provenance of semantic information in images to make them less susceptible to deep fake attacks. Our architecture includes semantic signing and verification steps. We apply this architecture to verifying two types of semantic information: individual identities (faces) and whether the photo was taken indoors or outdoors. Verification accounts for a collection of common image transformation, such as translation, scaling, cropping, and small rotations, and rejects adversarial transformations, such as adversarially perturbed or, in the case of face verification, swapped faces. Experiments demonstrate that in the case of provenance of faces in an image, our approach is robust to black-box adversarial transformations (which are rejected) as well as benign transformations (which are accepted), with few false negatives and false positives. Background verification, on the other hand, is susceptible to black-box adversarial examples, but becomes significantly more robust after adversarial training.

==> design.tex <==
\section{ImgProv Design Overview}

\section{End-to-End Image Provenance}

% \textcolor{blue}{Manav to describe the platform here}
% (signing and entire platform)

\section{Robustness of Property-based Signing}
% \textcolor{blue}{Mingyang to fill his design of system here}

% \textcolor{red}{\# 1. Figures' appearances still need to be improved}

% \textcolor{red}{\# 2. Currently I only tested downsampled images, do I need to run the experiments for brightness/contrast adjusted images?}

% \textcolor{red}{\# 3. Currently I only attack with epsilon==4, do I need to run the attack for other values of epsilon?}

% Deep convolutional networks are used to verify if the existing image and the input image is the same. For each input image, we first apply a multi-task cascaded convolutional network (MTCNN) to detect the face region and crop it out~\cite{DBLP:journals/corr/ZhangZL016}. After standardizing the cropped face image, we adjust it to a fixed size and feed it into an Inception-Resnet~\cite{DBLP:journals/corr/SzegedyIV16} to generate a 512-dimension feature vector. The cosine similarity between feature vectors of the input image and the existing image is then computed. Only if the cosine similarity is above a preset threshold will the pair of images be verified to be the same. 

% The key part of the above-mentioned pipeline is to train an Inception-Resnet network so that it can produce facial features of an image similar to its normally edited version, while producing different facial features for images of two individuals. Currently many common image editing operations are used, such as downsampling, color, brightness and contrast adjustment, as illustrasted in Figure \ref{fig:adjusted}. Since the difference between two different images of the same person is clearly greater than that of the two normally edited version of the same image, if the network can produce similar features for image pairs of the same person, it can definitely produce similar features for an image and its normally edited version. In order to make our model more robust to all possible image editing operations, we train the network to distinguish image pairs of the same person from those of different people.

% \begin{figure}[H]
% \begin{center}
% \includegraphics[width=25em]{figures/adjusted_visual_examples.png}
% \end{center}
%   \caption{Visual effects of common image editing operations}
% \label{fig:adjusted}
% \end{figure}

% During the training, immediately after the Inception-Resnet outputs a feature vector, we put that feature vector through a softmax classification layer to predict the identity of the input face image. The weights of the softmax classification layer are trained together with the rest of the weights by minimizing a cross-entropy loss function. When the trained model is used for inference, we remove the softmax classification layer from the network and directly output the feature vector. 
 
% To further test the robustness of our model, we generate adversarial examples by adding perturbation to images which is invisible to human eyes. The perturbed impersonator image is obtained by solving the following optimization problem: 

% \begin{equation}
% 	p(x) = x + \argmax\limits_{\bm{\delta}}\;\; \bm{sim}(f(\bm{x}+\bm{\delta}; \bm{\theta}), \bm{y}) 
% 	\;\;\;\;\; \text{s.t.} \;\;\lVert \bm{\delta} \rVert_{\infty}\leq  \epsilon
% \label{attack}
% \end{equation}

% where $\bm{sim}(\cdot)$ is the cosine similarity, $\bm{x}$ is the image used as the impersonator,
% $\bm{\delta}$ is the adversarial perturbation, $\bm{\theta}$ is the model parameter, $\bm{y}$ is the target image to be attacked.

% We perform both white-box and black-box Projected Gradient Descent attack (PGD attack)~\cite{DBLP:conf/iclr/MadryMSTV18}. More specifically, for a cropped target face image $\bm{y}$ of Person 1, we first randomly choose a cropped face image $\bm{x}$ of person 2 as the impersonator and resize $\bm{x}$ to match the dimensions of $\bm{y}$. Then we use PGD attack to add perturbation to the resized $\bm{x}$, and resize and standardize the perturbed $\bm{x}$ again to match the input dimensions of the network. Finally, we compute the similarity between the facial features of the 
% attack image $\bm{x}$ and the original image $\bm{y}$ to evaluate the effectiveness of the attack. We do 100 iterations of PGD attack with the step size of 0.2. The entire pipeline is illustrated in Figure \ref{fig:attack_pipeline}.

% \begin{figure}[H]
% \begin{center}
% \includegraphics[width=25em]{figures/attack_pipeline.png}
% \end{center}
%   \caption{Pipeline of adversarial attack}
% \label{fig:attack_pipeline}
% \end{figure}

% To defend our model from such attacks, we follow the approach by Madry et al. to finetune a pretrained model that is robust to adversarial attack~\cite{DBLP:conf/iclr/MadryMSTV18}. We define a new loss function inspired by the triplet loss~\cite{DBLP:conf/iclr/MadryMSTV18}. Given an input batch of image ${\{\bm{a_i}}\}_{i \in [1,2,..., n]}$, where $\bm{a_i}$ is a random image of the $i^{th}$ person, we find a second batch of image $\{\bm{p_i}\}_{i \in [1,2,..., n]}$, where $\bm{p_i}$ is also an image of the $i^{th}$ person but different from $\bm{a_i}$, and a third batch of image $\{\bm{n_i}\}_{i \in [1,2,..., n]}$, where $\bm{n_i}$ is an image of any person other than the $i^{th}$ person. While $\{\bm{a_i}\}$, $\{\bm{p_i}\}$, $\{\bm{n_i}\}$ are similar to the anchor image, positive image and negative image in the triplet loss, we split $\{\bm{n_i}\}$ into two halves: the first half $\{\bm{n_i}\}_{i \in [1,2,..., k]}$is composed of real negative images, and the second half $\{\bm{n_i}\}_{i \in [k+1,k+2,..., n]}$is composed of fake negative images perturbed by PGD attack. Then we define our new loss as the following:
% \begin{equation}
% % \begin{split}
% \begin{aligned}
% 	L(\{\bm{a_i}\}, \{\bm{p_i}\}, \{\bm{n_i}\}) =& \sum_{i=1}^{k} \bm{sim}(\bm{a_i}, \bm{n_i}) - \bm{sim}(\bm{a_i}, \bm{p_i})\;\; + \\
% 	&\sum_{i=k + 1}^{n} \bm{sim}(\bm{a_i}, p(\bm{n_i})) - \bm{sim}(\bm{a_i}, \bm{p_i})
% % \end{split}
% \end{aligned}
% \label{new_loss}
% \end{equation}

% By doing this, we hope that the training will make fake negative images dissimilar to their corresponding anchor images in terms of cosine similarity, while ensuring that real negative images still have the low similarity with anchor images as before.  During the adversarial training, we perform the same PGD attack as we do in testing. And in training we do 50 iterations of PGD attack with the step size of 0.2. 
